Graph Convolutional Networks with Dual Message Passing for Subgraph Isomorphism Counting and Matching

Graph neural networks (GNNs) and message passing neural networks (MPNNs) have been proven to be expressive for subgraph structures in many applications. Some applications in heterogeneous graphs require explicit edge modeling, such as subgraph isomorphism counting and matching. However, existing message passing mechanisms are not designed well in theory. In this paper, we start from a particular edge-to-vertex transform and exploit the isomorphism property in the edge-to-vertex dual graphs. We prove that searching isomorphisms on the original graph is equivalent to searching on its dual graph. Based on this observation, we propose dual message passing neural networks (DMPNNs) to enhance the substructure representation learning in an asynchronous way for subgraph isomorphism counting and matching as well as unsupervised node classification. Extensive experiments demonstrate the robust performance of DMPNNs by combining both node and edge representation learning in synthetic and real heterogeneous graphs. Code is available at https://github.com/HKUST-KnowComp/DualMessagePassing.

==> sections/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

==> sections/response.tex <==
\clearpage
\appendix

\section{General Response}
Thanks for the constructive reviews from all reviewers. We will improve this work based on your suggestions. The followings are responses to some unclear points. 

\subsubsection{Reproductivity}
We uploaded our code to CMT before the submission deadline of AAAI. We will publicly release the code and the processed data after this paper gets accepted. Detailed experimental settings will be also added in the extended pages.

\subsubsection{Motivation and Innovation}
Graph neural networks have been successfully applied in many fields, and this work follows the previous works to improve the neural subgraph counting and generalize to matching. Previous research studies show the feasibility in theory and practice. 
However, they did not completely solve the problem.
%But we still need to improve the capability of message passing. 
Our work is motivated by 
the one-to-one correspondence between isomorphisms in original graphs and isomorphisms in line graphs (described in the Whitney isomorphism theorem). Thus, we incorporate the line graph information into the message passing to enhance the structure learning. We introduce reversed edges associated with special edge types to ensure that (1) heterogeneous multigraphs and their line graphs also have the one-to-one mapping, (2) the numbers of isomorphisms (and subgraph isomorphisms) remain the same, and (3) the increased computation is still linear to the numbers of edges. We will clarify these in the abstract and introduction in the final copy version.

\subsubsection{Comparison with Prior Works}
%Due to the length limit, we pay little attention to the comparison between previous neural solutions and traditional algorithms. %Yangqiu: Don't draw attentions to negative effects.
Compared with the previous neural networks, we provide a theoretical guideline to model both node and edge representation and align them into the same embedding space. The motivation behind comes from isomorphisms so that the proposed DMPNN is suitable for subgraph isomorphism counting and matching as well as unsupervised structural learning. Some networks may also consider edge types, such as RGCN and HGT, and some variants also try to model edges as embeddings, such as CompGCN. However, they are not designed with such principles, and they may require additional more parameters and massive computation. 
% Traditional algorithms are hard to generalize to large patterns and large graphs, but neural networks can handle thanks to the linear complexity.
%We feel sorry for missing some related research, and we will give credit to these excellent works.
We will incorporate more references if the page limit allows.
%Yangqiu Never admit mistakes and say sorry in rebuttal.

\subsubsection{Efficiency}
In a message-passing framework, the computation cost is linear to the number of layers $K$ and edges $|E|$, i.e., $\mathcal{O}(K |E|)$. If we simply apply GNNs to the dual graph, the computation cost increases to $\mathcal{O}(K |E|^2)$. Our DMPNN does not explicitly construct the line graph but model edge representations with the dual graph property, shown in the ``Dual Message Passing Mechanism" subsection. Eq. (5) updates edge representation with the unoriented incidence matrix, which is a sparse matrix with $2 |E|$ non-zero elements. Thus, the proposed dual message passing is still $\mathcal{O}(K |E|)$, which is very efficient. Even adding reversed edges, the additional cost is still acceptable. We update the evaluation time in the following Table 7.
This running time comparison will be included in the latest version.

\begin{table}[!h]
    \tiny
    % \vspace{-0.1in}
    \centering
    \setlength\tabcolsep{1.5pt}
    % \resizebox{0.92\linewidth}{!}{%
    \begin{tabular}{l|ccccccccc}
    \toprule
    & CNN & LSTM & TXL & RGCN & RGIN & CompGCN & DMPNN & Deep-LRP & DMPNN-LRP \\
    \midrule
    Erd\H{o}s-Renyi & 7.86 & 8.88 & 8.74 & 1.44 & 1.51 & 6.37 & 5.90 & 7.23 & 7.50 \\
    Regular & 7.94 & 8.73 & 9.05 & 2.22 & 2.25 & 4.97 & 4.80 & 8.45 & 9.02 \\
    Complex & 36.55 & 38.16 & 39.17 & 7.98 & 8.14 & 31.32 & 29.55 & 34.12 & 35.19 \\
    MUTAG & 1.19 & 1.30 & 1.51 & 0.72 & 0.77 & 1.55 & 1.44 & 1.46 & 1.63 \\
    \bottomrule
    \end{tabular}
    \caption{Average time (in seconds) on test data in 100 runs.}
    \vspace{-0.2in}
\end{table}

% \subsubsection{Paper Organization}
% This work requires both graph theory and the background knowledge of message passing. Thus, some parts are not organized well. Overall, this draft starts from graph isomorphisms and the edge-to-vertex transform, introduces the one-to-one correspondence in isomorphisms between the original graph and its line graph, the carefully designed dual message passing, and its generalization to heterogeneous multigraphs. We will remove some redundancies to make the contents clearer.

\section{Response to Reviewer 1}
\subsubsection{Extendability}
The framework proposed by Liu et al. (2020) is to encode patterns and graphs separately and predict the counting with their representations. For multiple patterns with one single graph (e.g., knowledge graph queries) or one pattern with multiple graphs (e.g., social network mining), we can still encode these patterns and graphs individually and then predict counts or find matches of isomorphisms.
Moreover, we believe it is interesting to analyze temporal networks via pattern frequencies.

\section{Response to Reviewer 2}
\subsubsection{Content Organization}
Considering the researchers and readers with different background knowledge, we decided to involve all vital details in the main body. 
%But we agree there are some redundant preliminaries and propositions.
%There are some leaps between the connected contents, and we will improve the writing. 
%Yangqiu: I think it will be likely that only the meta-reviewer will briefly check the rebuttal. We cannot reveal our weakness by ourselves here.
Overall, our paper starts from graph isomorphisms and the edge-to-vertex transform, introduces the one-to-one correspondence in isomorphisms between one original graph and its line graph, proposes the carefully designed dual message passing, and generalizes it to heterogeneous multigraphs. We will improve the paper to make the contents clearer.

\subsubsection{Homogeneous vs. Heterogeneous}
The dual message passing depends on one-to-one correspondence between isomorphisms in original graphs and their line graphs. Sometimes, bijection does not hold. So we need to introduce the reversed edges with different specific edge types, which makes graphs heterogeneous. The message passing does not explicitly handle relation types but different types contribute to different initial edge embeddings. That is, our mechanism is appropriate for homogeneous and heterogeneous graphs (where \textit{Erd\H{o}s-Renyi} and \textit{Regular} are homogeneous). Considering the new edges are different with existing edges, the number of isomorphisms and subgraph isomorphisms remain the same (proof shown in Appendix B).

\section{Response to Reviewer 3}
\subsubsection{Isomorphism Illustration}
Thanks for your suggestion. Two same graphs only correspond to one particular isomorphism case. We will replace it with a complicated one.

\section{Response to Reviewer 4 \& 6}
\subsubsection{Experimental Details}
As subgraph isomorphism counting and matching are NP-complete, we regard them as regression problems by optimizing MSE jointly. The average of 3 trials on MSE is not better suited. 
%Yangqiu Please check if my modification is correct.
The ground truth is calculated by the VF2 algorithm. Thus, increasing the pattern size and the graph size is challenging to it. $\mathcal{X}_p$ and  $\mathcal{Y}_{p}$ stand for the node label set and edge label set, and we can observe significant gains across homogeneous and heterogeneous data.

